Adaptively Secure Coin-Flipping, Revisited

The full-information model was introduced by Ben-Or and Linial in 1985 to study collective coin-flipping: the problem of generating a common bounded-bias bit in a network of $n$ players with $t=t(n)$ faults. They showed that the majority protocol can tolerate $t=O(\sqrt n)$ adaptive corruptions, and conjectured that this is optimal in the adaptive setting. Lichtenstein, Linial, and Saks proved that the conjecture holds for protocols in which each player sends a single bit. Their result has been the main progress on the conjecture in the last 30 years. In this work we revisit this question and ask: what about protocols involving longer messages? Can increased communication allow for a larger fraction of faulty players? We introduce a model of strong adaptive corruptions, where in each round, the adversary sees all messages sent by honest parties and, based on the message content, decides whether to corrupt a party (and intercept his message) or not. We prove that any one-round coin-flipping protocol, regardless of message length, is secure against at most $\tilde{O}(\sqrt n)$ strong adaptive corruptions. Thus, increased message length does not help in this setting. We then shed light on the connection between adaptive and strongly adaptive adversaries, by proving that for any symmetric one-round coin-flipping protocol secure against $t$ adaptive corruptions, there is a symmetric one-round coin-flipping protocol secure against $t$ strongly adaptive corruptions. Returning to the standard adaptive model, we can now prove that any symmetric one-round protocol with arbitrarily long messages can tolerate at most $\tilde{O}(\sqrt n)$ adaptive corruptions. At the heart of our results lies a novel use of the Minimax Theorem and a new technique for converting any one-round secure protocol into a protocol with messages of $polylog(n)$ bits. This technique may be of independent interest.

==> abstract.tex <==
\iffalse
The question of how much bias a coalition of faulty players can
introduce into distributed sampling protocols in the full information model
was first studied by Ben-Or and Linial in 1985.
They focused on the problem of \emph{collective coin-flipping}, in which
a set of $n$ players wish to use their private
randomness to generate a common random bit $b$ in the presence of $t(n)$ faulty players, such that
the probability that $b=0$ (and 1) are at least $\eps$ for some
constant $\eps>0$. They showed that the majority function 
can tolerate $t=\Theta (\sqrt n)$ corruptions even in the presence of adaptive adversaries
and conjectured that this is optimal in the adaptive setting. Shortly thereafter, 
Lichtenstein, Linial, and Saks proved that the conjecture holds for protocols
where each player sends a single bit. 
Their result has been the main progress on the conjecture for the last 30 years.

\smallskip

In this work we revisit this question, and ask: what about protocols where players can send longer 
messages? Can increased communication enable tolerance of a larger fraction of corrupt players?

\smallskip

We introduce a model of \emph{strong adaptive} corruptions, in which an adversary sees all messages sent by honest parties in any given round, 
and based on the message content, decides whether to corrupt a party (and alter its message) or not. This is 
in contrast to the (classical) adaptive adversary, who corrupts parties based on prior communication history, and cannot alter messages already sent. 
Such strongly adaptive corruptions seem to be a realistic concern in settings where malicious parties can alter  
(or sabotage the delivery) of honest messages depending on their content, yet existing adversarial models do not take this into account.
We prove that any one-round coin-flipping protocol, \emph{regardless of message length}, 
can be secure against at most $\widetilde{O}(\sqrt n)$ strong adaptive corruptions. Thus, increased message length does not help in this setting.

\smallskip

We then shed light on the connection between adaptive and strongly adaptive adversaries, by proving
that for any symmetric one-round coin-flipping protocol secure against
$t$ adaptive corruptions, there is a symmetric one-round coin-flipping protocol
secure against $t$ strongly adaptive corruptions.
Going back to the standard adaptive model, we can now prove that any symmetric one-round protocol with arbitrarily long messages can tolerate at most $\widetilde{O}(\sqrt n)$
adaptive corruptions.

\smallskip

At the heart of our results there is a new technique for converting
any one-round secure protocol with arbitrarily long messages into a secure 
one where each player sends only $\polylog(n)$ bits.
This technique may be of independent interest.
\fi
The full-information model was introduced by Ben-Or and Linial in 1985 to study collective coin-flipping:
the problem of generating a common bounded-bias bit in a network of $n$ players with $t=t(n)$
faults. They showed that the majority protocol, in which each player sends a random bit and the output is the majority of the players' bits,
can tolerate $t(n)=O (\sqrt n)$ even in the presence of \emph{adaptive} corruptions,
and they conjectured  that this is optimal for such adversaries. 
Lichtenstein, Linial, and Saks proved that the conjecture holds for protocols
in which each player sends only a single bit. 
Their result has been the main progress on the conjecture during the last 30 years.

\medskip

In this work we revisit this question and ask: what about protocols where players can send longer 
messages? Can increased communication enable tolerance of a larger fraction of corrupt players?

\medskip


We introduce a model of \emph{strong adaptive} corruptions, in which an adversary sees all messages sent by honest parties in any given round and, based on the message content, decides whether to corrupt a party (and alter its message or sabotage its delivery) or not. This is 
in contrast to the (classical) adaptive adversary who can corrupt parties only based on past messages, and cannot alter messages already sent. 

\medskip

We prove that any one-round coin-flipping protocol, \emph{regardless of message length}, 
can be secure against at most $\widetilde{O}(\sqrt n)$ strong adaptive corruptions. Thus, increased message length does not help in this setting.

\medskip

We then shed light on the connection between adaptive and strongly adaptive adversaries, by proving
that for any symmetric one-round coin-flipping protocol secure against
$t $ adaptive corruptions, there is a symmetric one-round coin-flipping protocol
secure against $t$ strongly adaptive corruptions.
Going back to the standard adaptive model, we can now prove that any symmetric one-round protocol with arbitrarily long messages can tolerate at most $\widetilde{O}(\sqrt n)$
adaptive corruptions. 

\medskip

At the heart of our results there is a novel use of the Minimax Theorem and a new technique for converting
any one-round secure protocol  with arbitrarily long messages into a secure 
one where each player sends only  $\polylog(n)$ bits.
This technique may be of independent interest.

==> related-work.tex <==
\subsection{Related work}\label{related-work}

The full-information model (also known as the \emph{perfect information model}) was introduced by Ben-Or and Linial \cite{BL85} 
to study the problem of collective coin-flipping when no secret communication is possible between honest players.

\paragraph{In the static setting.}
Protocols for collective coin-flipping in the presence of static corruptions have been constructed in a series of works %\cite{BL85,AL93,AN93,Fei99,RZ01,RSZ02}
that variously focus on improving the fault-tolerance, round complexity, and/or bias of the output bit.
Feige \cite{Fei99} gave a protocol that is $(\delta^{1.65}/2)$-secure\footnote{A
coin-flipping protocol is $\eps$-secure against~$t$ static corruptions if for any static adversary that corrupts up to~$t$ parties, 
the probability that the protocol outputs~$0$ is at least $\eps$.}
in the presence of $t=(1+\delta)\cdot n/2$ static corruptions for any constant $0<\delta<1$.
Russell, Saks, and Zuckerman \cite{RSZ02} then showed that any protocol that is secure in the presence of linearly many corruptions must
either have at least $(1/2-o(1))\cdot\log^*(n)$ rounds, or communicate many bits per round.

Interestingly, nearly all proposed \emph{multi-round} protocols for collective coin-flipping
first run a \emph{leader election} protocol in which one of the $n$ players is selected as a ``leader'', who then outputs a bit that is taken as the protocol outcome.
We remark that this approach is inherently unsuitable for adaptive adversaries, which can always corrupt the leader after he is elected, 
and thereby surely control the protocol outcome.

\paragraph{In the adaptive setting.}
The study of coin-flipping protocols has been predominantly in the static setting.
The problem of adaptively secure coin-flipping was introduced by Ben-Or and Linial \cite{BL85}
and further examined by Lichtenstein, Linial, and Saks \cite{LLS89} as described in the previous section.
In addition, Dodis \cite{Dod00} proved that through ``black-box'' reductions from \emph{non-adaptive} coin-flipping, it is not possible to tolerate
significantly more corruptions than the majority protocol. The definition of ``black-box'' used in \cite{Dod00}
is rather restricted: it only considers sequential composition of non-adaptive coin-flipping protocols, followed by a (non-interactive)
function computation on the coin-flips thus obtained.

\paragraph{In the pairwise-channels setting.}
An adversarial model bearing some resemblance to our strong adaptive adversary model was introduced and analyzed by Hirt and Zikas \cite{HZ10}
in the \emph{pairwise communication channels} model, rather than the full-information model. In their model, the adversary can corrupt a party $P$ based on
some of the messages that $P$ sends within a round, then the adversary controls the rest of $P$'s messages in that round (and for future rounds).
Unlike in our strong adaptive model, the adversary of \cite{HZ10} cannot ``see inside all players' heads'' 
and overwrite arbitrary honest messages based on their content before they are sent.

\medskip

A brief survey of the literature on coin-flipping in the setting of computationally bounded players 
is given in Appendix \ref{appx:computationalSetting} due to space constraints.
